Asynchronous BFT Asset Transfer: Quasi-Anonymous, Light, and Consensus-Free

This paper introduces a new asynchronous Byzantine-tolerant asset transfer system (cryptocurrency) with three noteworthy properties: quasi-anonymity, lightness, and consensus-freedom. Quasi-anonymity means no information is leaked regarding the receivers and amounts of the asset transfers. Lightness means that the underlying cryptographic schemes are \textit{succinct} (\textit{i.e.}, they produce short-sized and quickly verifiable proofs) and each process only stores its own transfers while keeping communication cost as low as possible. Consensus-freedom means the system does not rely on a total order of asset transfers. The proposed algorithm is the first asset transfer system that simultaneously fulfills all these properties in the presence of asynchrony and Byzantine processes. To obtain them, the paper adopts a modular approach combining a new distributed object called ``agreement proof'' and well-known techniques such as commitments, universal accumulators, and zero-knowledge proofs.

==> alg/CFGKN20.tex <==
\begin{algorithm}[!tb]
\small
\caption{Scheme of the vector commitments in~\cite{CFGKN20}.}
\label{alg:CFGKN20}

\SpacedCommentLine{$\mathsf{Shamir\_Trick}$ computes an $(h_ih_j)$-root of $A$ using an $h_i$-root and an $h_j$-root of $A$~\textup{\cite{S83}}.}
\Operation{$\mathsf{Shamir\_Trick}(S_i,S_j,h_i,h_j)$}{
    $a,b \leftarrow \mathsf{Bezout}(h_i,h_j)$; \\
    \return $S_i^b S_j^a$.
}
\AlgoSkip

\Operation{$\comSetup(\lambda,l,n)$}{
    Generate a descriptor $\mathcal{G}\gets (\mathbb{G},g)$ for a group of unknown order; \\
    $A \leftarrow g^{\prod_{i=1}^n H_{\Primes}(i)}$; \Comment*{$A$ behaves as an accumulator digest for the primes $H_{\Primes}(i)$.} 
    \return $pp \leftarrow (\mathcal{G},A)$.
}
\AlgoSkip

\Operation{$\vccom_{pp}(v_1,...,v_n)$}{
    $\Forall i \in [n]$, compute $S_i \leftarrow g^{\prod_{j=1,j \neq i}^n H_{\Primes}(j)}$; \\
    $C \leftarrow S_1^{v_1}...S_n^{v_n}$; \\
    \return $C, aux \leftarrow (v_1,...,v_n)$.
}
\AlgoSkip

% \Operation{$\vcopen_{pp}(\Vec{I}, \Vec{v} ,\Vec{aux})$}{
%     $\Forall i \in [n]$, compute $S_i \leftarrow g^{\prod_{j=1,j \neq i}^n H_{\Primes}(j)}$; \\
%     $\pi_i \leftarrow \sqrt[H_{\Primes}(i)]{\prod_{j=1,j \neq i}^n S_j^{v_j}} \mod{N}$; \\
%     \return $\pi_i$.
% }

\Operation{$\vcopen_{pp}(v,i,aux)$}{
    $\Forall k \in [n]$, compute $S_{i,k} \leftarrow g^{\prod_{j=1,j \neq i, j \neq k}^n H_{\Primes}(j)}$; \\
    % $\pi_i \leftarrow \sqrt[H_{\Primes}(i)]{\prod_{j=1,j \neq i}^n S_j^{v_j}} \mod{N}$; \\
    $\pi_i \leftarrow \prod_{j=1,j \neq i}^n S_{i,j}^{v_j}$; \\
    \return $\pi_i,S_i$;
}

\AlgoSkip

\Operation{$\vcver_{pp}(C,v,i,S_i,\pi_i)$}{
    $h_i \leftarrow H_{\Primes}(i)$; \\
    \return $A = S_i^{h_i} \land C = S_i^v\pi_i^{h_i}$; \Comment*{$S_i$ behaves as an accumulator proof of membership for $h_i$.}
}

\AlgoSkip

\Operation{$\vcup_{pp}(C,v,v',S_i,i)$}{
    $\Assert(A = S_i^{H_{\Primes}(i)})$; \\
    $C' \leftarrow C \cdot S_i^{v'-v}$; \\
    $U \leftarrow (v,v',S_i,i)$; \\
    \return $C',U$;
}

\AlgoSkip

\Operation{$\vcpup_{pp}(C,j,\pi_j, S_j, U)$}{
    $v,v',S_i,i \leftarrow U$; \\
    $h_i \gets H_{\Primes}(i)$; \\
    $h_j \gets H_{\Primes}(j)$; \\
    $\Assert(A = S_i^{h_i})$; \\
    \lIf{$i = j$}{
        \return $\pi_j$
    }
    \lElse{
        \return $\pi_j \cdot \mathsf{ShamirTrick}(S_i,S_j,h_i,h_j)^{v'-v}$;
    }
}

% \Operation{$\vcup_{pp}(C,v,v',i)$}{
%     $C' \leftarrow C \cdot S_i^{v'-v}$; \\
%     $U \leftarrow (v,v',i)$; \\
%     \return $C,U$.
% }
% \AlgoSkip

% \Operation{$\vcpup_{pp}(C,\pi_j, v', i, U)$}{
%     \lIf{$i = j$}{
%         \return $\pi_j$;
%     }
%     \lElse{
%         \return $\pi_j \sqrt[H_{\Primes}(j)]{S_i^{v'-v}}$.
%     }
% }

% \Operation{$\vcgen(k,l,n)$}{
%     $p,q \leftarrow \mathsf{Primes}(k/2)$; \\
%     $N \leftarrow pq$; \\
%     $g \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathbb{Z}_N$; \\
%     $A \leftarrow g^{\prod_{i=1}^n H(i)}$; \\
%     \return $pp \leftarrow (N,g,A)$;
% }

% \Operation{$\vccom_{pp}(v_1,...,v_n)$}{
%     \For{$i \in [n]$}{
%         $S_i \gets g^{\prod_{j=1,j \neq i}^n h_j}$;
%     }
%     $C \leftarrow S_1^{v_1}...S_n^{v_n}$; \\
%     \return $C, aux \leftarrow (v_1,...,v_n)$;
% }

% \Operation{$\vcopen_{pp}(v,i,aux)$}{
%     \For{$k \in [n]$}{
%         $S_k \gets g^{\prod_{j=1,j \neq k}^n h_j}$;
%     }
%     $\pi_i \leftarrow \sqrt[h_i]{\prod_{j=1,j \neq i}^n S_j^{v_j}} \mod{N}$; \\
%     \return $\pi_i,S_i$;
% }

% \Operation{$\vcver_{pp}(C,v,i,S_i,\pi_i)$}{
%     $h_i \leftarrow H(i)$; \\
%     \return $A = S_i^{h_i} \land C = S_i^v\pi_i^{h_i}$;
% }

% \Operation{$\vcup_{pp}(C,v,v',S_i,i)$}{
%     $\Assert(A = S_i^{H(i)})$; \\
%     $C' \leftarrow C \cdot S_i^{v'-v}$; \\
%     $U \leftarrow (v,v',S_i,i)$; \\
%     \return $C',U$;
% }

% \Operation{$\vcpup_{pp}(C,j,\pi_j, S_j, h_j, U)$}{
%     $h_i \gets H(i)$; \\
%     $\Assert(A = S_i^{h_i})$; \\
%     \lIf{$i = j$}{
%         \return $\pi_j$
%     }
%     \lElse{
%         \return $\pi_j \cdot \mathsf{ShamirTrick}(S_i,S_j,h_i,h_j)^{v'-v}$;
%     }
% }

\end{algorithm}

==> alg/Global_VC.tex <==
\begin{algorithm}[!tb]
\small
\caption{Variant with concurrent updates of the VC scheme of~\cite{CFGKN20}}
\label{alg:shared}

\SpacedCommentLine{$\comIndSetup$ is called by each process to compute their personal data.}
\Operation{$\comIndSetup_{pp}(i)$}{
    $S_i \leftarrow g^{\prod_{j=1,j \neq i}^n H_{\Primes}(j)}$; \\
    $h_i \leftarrow H_{\Primes}(i)$; \\
    $v_i \leftarrow 0$; \\
    $C \leftarrow 1$; \Comment*{The committed vector is initially empty.}
    \return $sp_i \leftarrow (S_i,h_i,v_i,C)$;
}

\AlgoSkip

\Operation{$\comCommut_{pp,sp_i}(S_j,v)$}{
    $\Assert(A = S_j^{H_{\Primes}(j)})$; \\
    $S_{i,j} \leftarrow \mathsf{ShamirTrick}(S_i,S_j,i,j)$; \\
    $a,b \leftarrow \mathsf{Bezout}(v_i,v)$; \\
    \return $C^b = (S_{i,j}^{v_ia} \pi_i^b S_{i,j}^{-\mathsf{GCD}(v_i,v)})^{H_{\Primes}(i)}(S_i^{v_i}S_j^{v})^b$;\label{line:verif}
}

\AlgoSkip

\Operation{$\comCommup_{pp,sp_i}(C',j,S_j,v,v',\pi_j)$}{
    $\Assert(i \neq j \land \vcver_{pp}(C',v,j,S_j,\pi_j))$; \\
    \lIf{$C \neq C'$}{
        $\Assert(\comCommut_{pp,sp_i}(S_j,v))$;
    }
    $C \leftarrow \vcup_{pp}(C,v,v',S_j,j)$; \\
    $\pi_i \leftarrow \vcpup_{pp}(C,j,\pi_j, S_j, U)$;\\
    \return $C,\pi_i$; \\
}

\end{algorithm}

==> alg/NIPoKCR.tex <==
\SetKwHangingKw{Params}{params:}
\SetKwHangingKw{Inputs}{inputs:}
\SetKwHangingKw{Witness}{witness:}
\SetKwHangingKw{Claim}{claim:}

\begin{algorithm}[H]
        \Params{$\mathbb{G} \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{GGen}(\lambda)$; $\aangle{g_1, g_2} \in \mathbb{G}$;}
        \Inputs{$e \in \mathbb{Z}$; $X \leftarrow g_1^x \in \mathbb{G}$; $L \leftarrow g_2^\ell \in \mathbb{G}$; $\ell_e \leftarrow H_\Primes(H(e)) \in \Primes(s_1,s_2)$;}
        \Witness{$x \in \mathbb{Z}$; $\ell \in \mathbb{G}$;}
        \Claim{$x \equiv e \mod{\ell_e} \land \ell_e \mid \ell$.}
        
        Prover computes $q_e, r_e$  and $q_x, r_x$ s.t. $e=q_e \ell_e + r_e$ and $x=q_x \ell_e + r_x$; 
        Prover computes $q_\ell$ s.t. $\ell=\ell_e q_\ell$;
        Prover sends $Q_1 \leftarrow g_1^{q_x} g_2^{q_e}$ and $Q_2 \leftarrow g_2^{q_\ell}$ to Verifier; \\
        
        Verifier computes $r_e = e \mod{\ell_e}$ and accepts if $Q_1^{\ell_e}(g_1 g_2)^{r_e} = X g_2^e \land Q_2^{\ell_e}=L$.
        
    \caption{Non-Interactive Proof of Knowledge of Chinese Remainder (NIPoKCR).}
    \label{alg:NIPoKCR}
\end{algorithm}

==> alg/NIPoKNCR.tex <==
\SetKwHangingKw{Params}{params:}
\SetKwHangingKw{Inputs}{inputs:}
\SetKwHangingKw{Witness}{witness:}
\SetKwHangingKw{Claim}{claim:}

\begin{algorithm}[H]
        \Params{$\mathbb{G} \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{GGen(\lambda)}$; $\aangle{g_1, g_2} \in \mathbb{G}$;}
        \Inputs{$e \in \mathbb{Z}$; $X \leftarrow g_1^x \in \mathbb{G} $; $L \leftarrow g_2^\ell \in \mathbb{G}$;$\ell_e \leftarrow H_{\Primes}(H(e)) \in \Primes(s_1,s_2)$;}
        \Witness{$x \in \mathbb{Z}$; $\ell \in \mathbb{G}$;}
        \Claim{$x \not\equiv e \mod{\ell_e} \lor \ell_e \nmid \ell$.}
    
        If $\ell_e \nmid \ell$, then Prover computes the Bezout coefficient $a,b$ s.t. $a\ell + b\ell_e=1$ and sends $a$ and $B=g_2^b$;
        
        Else Prover determines $q_e, r_e$  and $q_x, r_x$ s.t. $e=q_e \ell_e + r_e$ and $x=q_x \ell_e + r_x$, then computes $Q_x=g_1^{q_x}$, $R_x=g_1^{r_x}$, $Q_e=g_2^{q_e}$ and a range proof $\pi$ for $R_x$ proving that $r_x \in [\ell_e]$ and sends $Q_x,R_x,Q_e$ and $\pi$ to Verifier;
        
        Verifier accepts if $L^a B^{\ell_e}=g_2$ or computes $r_e = e \mod{\ell_e}$ and accepts if $\pi$ is a valid range proof for $R_x$ and $X g_2^{e} = Q_x^{\ell_e} R_x Q_e^{\ell_e}+g_2^{r_e} \land R_x \neq g_1^{r_e}$.
    \caption{Non-Interactive Proof of Knowledge of Non-Chinese Remainder (NIPoKNCR).}
    \label{alg:NIPoKNCR}
\end{algorithm}

==> alg/PoKCR.tex <==
\SetKwHangingKw{Params}{params:}
\SetKwHangingKw{Inputs}{inputs:}
\SetKwHangingKw{Witness}{witness:}
\SetKwHangingKw{Claim}{claim:}

\begin{algorithm}[H]
    \label{alg:PoKCR}

        \Params{$\mathbb{G} \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{GGen(\lambda)}$; $\aangle{g_1,g_2} \in \mathbb{G}$;}
        \Inputs{$e \in \mathbb{Z}$;}
        \Witness{$x \in \mathbb{Z}$;}
        \Claim{$x \equiv e \mod{l_e}$.}
        Prover sends $X \leftarrow g_1^x$ to Verifier; \\
        Verifier sends $l_e$ to Prover; \\
        Prover computes $q_e, r_e$  and $q_x, r_x$ s.t. $e=q_el_e + r_e$ and $x=q_xl_e + r_x$;
        Prover sends $Q \leftarrow g_1^{q_x}g_2^{q_e}$ and $r_e$; \\
        Verifier accepts if $ r_e \in [l_e]$ and $Q^{l_e}(g_1g_2)^{r_e} = X g_2^e$;

        
    \caption{Proof of Knowledge of Chinese Remainder (PoKCR)}
\end{algorithm}

==> alg/PoKRep.tex <==
\SetKwHangingKw{Params}{params:}
\SetKwHangingKw{Inputs}{inputs:}
\SetKwHangingKw{Witness}{witness:}
\SetKwHangingKw{Claim}{claim:}

\begin{algorithm}[H]
        \Params{$\mathbb{G} \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{GGen(\lambda)}$; $(g_1,...,g_n) \in \mathbb{G}^n$;}
        \Inputs{$w \in \mathbb{G}$;}
        \Witness{$\bm{x} \in \mathbb{Z}^n$;}
        \Claim{$\mathsf{Rep}(x) = \prod_{i=1}^{n}g_i^{x_i} = w$;}
        Verifier sends $\ell \overset{{\scriptscriptstyle\$}}{\leftarrow} \Primes(2,\lambda)$; \\
        For each $x_i$, Prover finds $q_i, r_i$ s.t. $x_i = q_i \ell + r_i$, sets $\bm{q} \leftarrow \aangle{q_1,...,q_n} \in \mathbb{Z}^n$ and $\bm{r} \leftarrow \aangle{r_1,...,r_n} \in [\ell]^n$; Prover sends $Q \leftarrow \prod_{i=1}^{n}g_i^{q_i}$ and $\bm{r}$ to Verifier; \\
        Verifier accepts if $\bm{r} \in [\ell]^n$ and $Q^\ell \mathsf{Rep}(r) = w$.

    \caption{Proof of Knowledge of Representation (PoKRep)~\cite{BBF19}.}
    \label{alg:PoKRep}
\end{algorithm}

==> alg/crasse.tex <==
\begin{algorithm}
\Operation{$\AccSetup(\lambda)$}{
    $\mathcal{G}=\aangle{\mathbb{G},A,B} \leftarrow \mathsf{GGen}(\lambda)$; \\
    $\aangle{g_1,g_2} \leftarrow \mathcal{O}_1$; \\
    Setup $H_\Primes$ with prime domain $\Primes(b_2,b_1)$; \\ 
    $v_0,\ell_0 \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathbb{Z}^+ \times \Primes(b_1+1,b)$ ; \Comment{Sample a random prime initial value} 
    $sp \leftarrow \aangle{v_0,\ell_0}$; \\
    $A_0 \leftarrow \aangle{g_1^{v_0},g_2^{\ell_0}}$; \\
    $pp \leftarrow \aangle{\mathcal{G}, g_1, g_2, H_\Primes, A_0}$; \\
    \return $\aangle{pp,sp,A_0}$.
}
\AlgoSkip

\Operation{$\accAdd(pp,sp,A,v)$}{
    \lIf{$\accProveMem(pp,sp,A,v) \neq \abort$}{\return $A$;}
    $\aangle{\mathcal{G}, g_1, g_2, H_\Primes} \leftarrow pp$; \\
    $\aangle{x,\ell} \leftarrow sp$; \\
    $\ell_v \leftarrow H_{\Primes}(H(v))$; \\
    Solve the CRT for $x' \equiv x \mod{\ell}$ and $x' \equiv v \mod{\ell_v}$; \\
    $\ell' \leftarrow \ell \times \ell_v$; \\
    $sp \leftarrow \aangle{x',\ell'}$; \\
    $A \leftarrow \aangle{g_1^{x'},g_2^{\ell'}}$; \\
    \return $\aangle{sp,A}$.
}
\AlgoSkip

\Operation{$\accDel(pp,sp,A,v)$}{
    \lIf{$\accProveNonMem(pp,sp,A,v) \neq \abort$}{\return $A$;}
    $\aangle{\mathcal{G}, g_1, g_2, H_\Primes} \leftarrow pp$; \\
    $\aangle{x,\ell} \leftarrow sp$; \\
    $\ell_v \leftarrow H_{\Primes}(H(v))$; \\
    $\ell' \leftarrow \ell / \ell_v$; \\
    $x' \leftarrow x \mod{\ell'}$; \\
    $sp \leftarrow \aangle{x',\ell'}$; \\
    $A \leftarrow \aangle{g_1^{x'},g_2^{\ell'}}$; \\
    \return $\aangle{sp,A}$.
}
\AlgoSkip

\Operation{$\accProveMem(pp,sp,A,v)$}{
    \return $\NIPoKCR_\mathsf{prove}(pp,sp,A,v)$.
}
\AlgoSkip

\Operation{$\accProveNonMem(pp,sp,A,v)$}{
    \return $\NIPoKNCR_\mathsf{prove}(pp,sp,A,v)$.
}
\AlgoSkip

\Operation{$\accVerifyMem(pp,A,v,w)$}{
    \return $\NIPoKCR_\mathsf{verify}(pp,A,v,w)$.
}
\AlgoSkip

\Operation{$\accVerifyNonMem(pp,A,v,u)$}{
    \return $\NIPoKCR_\mathsf{verify}(pp,A,v,u)$.
}
\caption{Chinese-remainder-based accumulator with sublinear storage (CRASSe).}
\label{alg:CRASSe}
\end{algorithm}

==> alg/zkPokRep.tex <==
\SetKwHangingKw{Params}{params:}
\SetKwHangingKw{Inputs}{inputs:}
\SetKwHangingKw{Witness}{witness:}
\SetKwHangingKw{Claim}{claim:}

\begin{algorithm}[H]
    \label{alg:zkPoKRep}
        \Params{$\mathbb{G} \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{GGen(\lambda)}$; $(g_1,...,g_n) \in \mathbb{G}^n$; $B > 2^{2\lambda}$;}
        \Inputs{$w \in \mathbb{G}$;}
        \Witness{$\textbf{x} \in \mathbb{Z}^n$;}
        \Claim{$\mathsf{Rep(x)} = \prod_{i=1}^{n} g_i^{x_i} = w$;}
        Prover chooses random $k_1,...,k_n \overset{{\scriptscriptstyle\$}}{\leftarrow} [-B,B]$, sends $A=\prod_{i=1}^{n} g_i^{k_i}$ to Verifier; \\
        Verifier sends $c \overset{{\scriptscriptstyle\$}}{\leftarrow} [0,2^\lambda]$ and $l \overset{{\scriptscriptstyle\$}}{\leftarrow} \mathsf{Primes}(\lambda)$; \\
        Prover computes $s_i=k_i + c x_i$ and then derives quotients $\textbf{q}\in \mathbb{Z}^n$ and residues $\textbf{r} \in [l]^n$ s.t. $q_i*l_i+r_i=s_i$; Prover sends $Q = \prod_{i=1}^n g_i^{q_i}$ and $\textbf{r}$ to the Verifier.
        Verifier accepts if $r_i \in [l]$ and $Q^l \prod_{i=1}^{n} g_i^{r_i} = Aw^c$ 
                
    \caption{Zero-knowledge Proof of Knowledge of Representation (ZKPoKRep)~\cite{BBF19}}
\end{algorithm}

==> at-sequenciality-proof-TA.tex <==
%% 2024_09_23 FT: Earlier proof of AT-Sequentiality, before Maxence's remark and scenario

\mparagraph{Method $M$ for constructing an invocation sequence $S$.}
\newcommand{\porder}{\rightarrow_I}
\newcommand{\set}{\mathsf{set}}
\ft{For any execution of \Cref{alg:aat} in which correct processes execute the local histories $\{L_i\}_{p_i\in C}$ (where $C$ is the set of correct processes), we use the following construction to exhibit a mock global $H$ that respect the AT-properties (\Cref{sec:amt-spec}).

This construction relies on the following notation:
\begin{itemize}
    \item If $o_i$ is some invocation 
\end{itemize}

We define recursively the following set $I$ of invocations and the relation $\porder$ on $I$.
\begin{itemize}
    \item $I$ contains all the $\transfer_i(v,j)$ and $\balance_i()$ operation invocations by correct processes $p_i\in C$.
    $$I=\bigcup_{p_i\in C} \set(L_i),$$
    where $\set(L_i)$ denotes the elements contained in the sequence $L_i$.
    \FT{Work in progress \todo{To be continued}}
\end{itemize}


}
We describe in the following a method, that we call $M$, for constructing a sequence $S$ of all the operation invocations produced by an execution of \Cref{alg:aat}, captured as a global history $H=(L_1,...,L_n)$.
First, we incrementally construct a partially-ordered set (poset) $P=(I,\porder)$, where $I$ is the set of all operation invocations of the execution and $\porder$ is a partial order on $I$ defining the precedence of invocations.
Initially, for every correct process $p_i$, $I$ includes all the $\transfer_i(v,j)$ and $\balance_i()$ operation invocations in $L_i$, and the $\porder$ order extends the $\rightarrow_i$ process order.
We also define a set called $\mathit{receiving\_APs\_to\_process}$, which contains non-null receiving APs that must be processed to construct $P$.
Non-null receiving APs are particularly important, as they allow us to infer $\porder$ relations between the $\transfer()$ invocations of different processes.
The $\mathit{receiving\_APs\_to\_process}$ set is initialized with all non-null receiving APs produced during the execution by correct processes at \cref{line:aat-process-create-ap}, in a $\prove()$ call at \cref{line:aat-rcv-trf-process}.
We now describe the steps to construct $P$ iteratively.
\begin{enumerate}
    \item We initialize a new variable $\mathit{new\_receiving\_APs}$ to the empty set $\varnothing$.
    This set will contain the new non-null receiving APs discovered during the current iteration, and it will replace the current $\mathit{receiving\_APs\_to\_process}$ at the end of the iteration.
    (Some non-null receiving APs can be ``rediscovered'' several times during the procedure, which does not pose a problem for the construction.)
    %(\ie $\mathit{new\_receiving\_APs} \gets \varnothing$).

    \item For every non-null receiving AP $\ap_\rcv^{\sn_\rcv} \in \mathit{receiving\_APs\_to\_process}$, we get the matching non-null sending AP $\ap_\snd^{\sn_\snd}$ and its associated sequence of previous APs $\mathit{previous\_APs}_\snd^{\sn_\snd}$, and execute the following sub-steps.
    \begin{enumerate}
        \item For every sending AP $\ap_\snd^{\sn_\snd'} \in \mathit{previous\_APs}_\snd^{\sn_\snd}$, we add its corresponding $\transfer_\snd^{\sn_\snd'}(\star,\star)$ invocation in $I$ if it was not already contained (typically because $p_\snd$ is correct).

        \item For every pair of invocations $o_\snd'=\transfer_\snd^{\sn_\snd'}(\star,\star), o_\snd''=\transfer_\snd^{\sn_\snd''}(\star,\star) \in I$ s.t. $\sn_\snd' < \sn_\snd''$, we have $o_\snd' \porder o_\snd''$ (process order of $p_\snd$).
    
        \item For every pair of invocations $o_\rcv'=\op_\rcv^{\sn_\rcv'}(), o_\snd'=\op_\snd^{\sn_\snd'}() \in I$ s.t. $\sn_\snd' \leq \sn_\snd$ and $\sn_\rcv \leq \sn_\rcv'$, we have $o_\snd' \porder o_\rcv'$ (the sending precedes the reception).
        % To also consider the cases where the sender and/or the receiver are correct processes with $\balance()$ invocations, we can also replace the $\transfer_\snd^{\sn_\snd'}(\star,\star) \in I$ by $\balance_\snd^{\sn_\snd'}() \in I$ and $\transfer_\rcv^{\sn_\rcv'}(\star,\star) \in I$ by $\balance_\rcv^{\sn_\rcv'}() \in I$ and reapply the same $\porder$ relation.

        % \item For every pair $\transfer_\snd^{\sn_\snd'}(\star,\star),\balance_\rcv^{\sn_\rcv'}() \in I$ s.t. $\sn_\snd' \leq \sn_\snd$ and $\sn_\rcv \leq \sn_\rcv'$, we have $\transfer_\snd^{\sn_\snd'}(\star,\star) \porder \balance_\rcv^{\sn_\rcv'}()$ (same as before, but for $\balance()$ invocations if the receiver is a correct process).
        
        \item We add all receiving APs of $\mathit{previous\_APs}_\snd^\sn$ to $\mathit{new\_receiving\_APs}$.
    \end{enumerate}

    \item We assign $\mathit{new\_receiving\_APs}$ to $\mathit{receiving\_APs\_to\_process}$.
    
    \item Repeat from step 1 until $\mathit{receiving\_APs\_to\_process}$ is empty.
\end{enumerate}

Once we have finished performing the above steps, we perform the transitive closure on the $\porder$ relation to make sure that we end up with a well-formed partial order.
\TA{Do we have to justify that we can apply a transitive closure on $\porder$? (ie $\porder$ had no cycle)}
\TA{To prove the absence of cycles in the graph of APs, we concluded with François that we need an additional assumption on the fact that if some proving scheme provides Knowledge-Soundness (eg, AP and ZKP), then for a given valid proof, the associated knowledge must have been known by the prover before the generation, otherwise it may be possible to create cycles of APs in our system. We also need to assume time "linearity"/asymmetry (it shouldn't be possible for two distinct events to precede each other). This assumption would capture "Knowledge-Soundness-Causality".}

% Once we have finished performing the above steps, we obtain a complete poset $P=(I,\porder)$ where $\porder$ is a strict partial order on $I$.
% \TA{Do we have to justify that the resulting $\porder$ is a partial order (no cycle and no need to apply a transitive closure?)}
Finally, we obtain a sequence $S$ containing all the invocations of $I$ by collapsing the $\porder$ partial order into any possible total order $\rightarrow_S$.

\TA{Maybe the spec does not guarantee liveness as is, \ie we do not guarantee that if a correct process transfers to another correct process, the funds are eventually received. Indeed, every \transfer that does not abort can be put at the end of the AT-sequence, which would still respect AT-Sequentiality. A way to guarantee liveness would be to say that, if the correct receiver does an infinite amount of operation invocations, then eventually it will ``see'' the funds that were sent to it. Maybe it is already guaranteed? If this is already guaranteed, what I find strange is that we never had to talk about the \send operation in the correctness proof to show that our algorithm is live.}

\atsequentiality*

\begin{proof}
Let us consider any execution of \Cref{alg:aat}, captured as a global history $H=(L_1,...,L_n)$.
We subsequently show that any sequence of invocation $S$ created from $H$ using method $M$ is an AT-sequence.
Let us consider one of such sequences that we call $S$, with $\rightarrow_S$ its associated total order.
We have the following for every operation invocation $o=\op_i^\sn() \in S$ by process $p_i$ at sequence number \sn.
\begin{itemize}
    \item Case where $o$ is a $\balance_i^\sn()/v$ invocation.
    In this case, $p_i$ is necessarily correct, and we have to prove that $v = \total(i,\{o' \in S \mid o' \rightarrow_S o\})$.
    
    By construction of $S$ using method $M$, the following holds.
    For all the $\transfer_i^{\sn'}(v',j)$ sent by $p_i$ before $o$ in $S$ where $i \neq j$, $p_i$ has subtracted $v'$ to its balance $\bal_i$ at \cref{line:aat-process-update-bal} during the $\prove()$ call at \cref{line:aat-trf-process}.
    Likewise, for all the $\transfer_j^{\sn'}(v',i)$ received by $p_i$ before $o$ in $S$ where $i \neq j$, $p_i$ has added $v'$ to its balance $\bal_i$ at \cref{line:aat-process-update-bal} during the $\prove()$ call at \cref{line:aat-rcv-trf-process}.
    Therefore, the value $v$ returned by $\balance_i^\sn()/v$ is computed exactly like $\total(i,\{o' \in S \mid o' \rightarrow_S o\})$.

    \item Case where $o$ is a $\transfer_i^\sn(v,j)$ invocation (remind that, implicitly, we only consider $\transfer()/r$ invocations that return $r=\commit$).
    In this case, we have to prove that $v \leq \total(i,\{o' \in S \mid o' \rightarrow_S o\})$.
    
    If the sender $p_i$ is correct, then the proof follows the same reasoning as the previous case, and from the fact that $p_i$ checks that it has enough funds for the transfer at \cref{line:aat-trf-check-bal}.
    
    If the sender $p_i$ is Byzantine, the proof relies on the \Pzk predicate.
    For each of the valid APs $\ap_i^{\sn'}$ at $\sn'$ from $p_i$ (where $0 < \sn' \leq \sn$) that are used to construct $S$ using method $M$, $p_i$ must provide in the \secdata of the associated ZKP $\zkp_i^{\sn'}$ its old and new balances, respectively denoted $\bal_\prover$ and $\bal_\prover'$ at \cref{line:pzk-secdata-unwrap}.
    Be $\ap_i^{\sn'}$ a null AP, a non-null sending AP, or a non-null receiving AP, the transition from the old to the new balance of $p_i$ is verified in zero-knowledge at \cref{line:pzk-check-snd-is-rcv}, \ref{line:pzk-check-pvr-is-snd}, or~\ref{line:pzk-check-pvr-is-rcv}, respectively.
    
    By construction of $S$ using method $M$, we have the following for each of the valid APs $\ap_i^{\sn'}$ at $\sn'$ from $p_i$ where $0 < \sn' < \sn$.
    If $\ap_i^{\sn'}$ is a sending AP corresponding to a $\transfer_i^{\sn'}(v',j)$ invocation, then $\transfer_i^{\sn'}(v',j)$ must appear before $o$ in the $\porder$ order.
    Likewise, if $\ap_i^{\sn'}$ is a receiving AP corresponding to a $\transfer_j^{\sn''}(v',i)$ invocation, then $\transfer_j^{\sn''}(v',i)$ must appear before $o$ in the $\rightarrow_S$ total order.
    Therefore, by induction, the balance of a Byzantine process is also computed exactly like $\total(i,\{o' \in S \mid o' \rightarrow_S o\})$.
    
    Finally, due to the $\bal_\prover \geq v$ check at \cref{line:pzk-check-pvr-is-snd}, the old balance of $p_i$ right before $o$ is guaranteed to be greater than transfer value, which concludes the proof.
    \TA{No mention of accumulator in the proof, is it strange?}
    \qedhere
\end{itemize}
\end{proof}

